Local moment matching with Erlang mixtures under automatic roughness penalization

We consider the class of Erlang mixtures for the task of density estimation on the positive real line when the only available information is given as local moments, a histogram with potentially higher order moments in some bins. By construction, the obtained moment problem is ill-posed and requires regularization. Several penalties can be used for such a task, such as a lasso penalty for sparsity of the representation, but we focus here on a simplified roughness penalty from the P-splines literature. We show that the corresponding hyperparameter can be selected without cross-validation through the computation of the so-called effective dimension of the estimator, which makes the estimator practical and adapted to these summarized information settings. The flexibility of the local moments representations allows interesting additions such as the enforcement of Value-at-Risk and Tail Value-at-Risk constraints on the resulting estimator, making the procedure suitable for the estimation of heavy-tailed densities.

==> assets/GaussRevGamma/1000/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,3.656[$ & 500 & 4 & 0.500 & 1.192 & 3.474 & 10.994 & 36.002 \\
2 & $[3.656,4.384[$ & 400 & 4 & 0.400 & 1.598 & 6.397 & 25.677 & 103.319 \\
3 & $[4.384,4.743[$ & 90 & 4 & 0.090 & 0.408 & 1.851 & 8.398 & 38.127 \\
4 & $[4.743,\infty[$ & 10 & 1 & 0.010 & 0.049 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/GaussRevGamma/1000/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{3.643} & \num{4.376} & \num{4.530} & \num{4.778} & \num{4.857} \\
Sample values & \num{3.656} & \num{4.384} & \num{4.532} & \num{4.743} & \num{4.840} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{3.612} & \num{4.489} & \num{4.736} & \num{5.213} & \num{5.392} \\
$\bm k = (2, 2, 2, 1)$ & \num{3.611} & \num{4.487} & \num{4.735} & \num{5.210} & \num{5.390} \\
$\bm k = (3, 3, 3, 1)$ & \num{3.612} & \num{4.488} & \num{4.735} & \num{5.213} & \num{5.393} \\
$\bm k = (4, 4, 4, 1)$ & \num{3.612} & \num{4.490} & \num{4.737} & \num{5.211} & \num{5.390} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.027} & \num{0.032} & \num{0.035} & \num{0.042} & \num{0.047} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.028} & \num{0.033} & \num{0.037} & \num{0.045} & \num{0.049} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.027} & \num{0.033} & \num{0.036} & \num{0.043} & \num{0.048} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.028} & \num{0.032} & \num{0.036} & \num{0.044} & \num{0.045} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.041} & \num{0.118} & \num{0.209} & \num{0.437} & \num{0.537} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.042} & \num{0.117} & \num{0.208} & \num{0.435} & \num{0.535} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.041} & \num{0.118} & \num{0.209} & \num{0.437} & \num{0.538} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.042} & \num{0.119} & \num{0.210} & \num{0.435} & \num{0.535} \\
\bottomrule 
\end{tabularx}


==> assets/GaussRevGamma/2000/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,3.641[$ & 1000 & 4 & 0.500 & 1.153 & 3.289 & 10.260 & 33.263 \\
2 & $[3.641,4.362[$ & 800 & 4 & 0.400 & 1.590 & 6.338 & 25.326 & 101.444 \\
3 & $[4.362,4.730[$ & 180 & 4 & 0.090 & 0.406 & 1.834 & 8.287 & 37.462 \\
4 & $[4.730,\infty[$ & 20 & 1 & 0.010 & 0.048 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/GaussRevGamma/2000/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{3.643} & \num{4.376} & \num{4.530} & \num{4.778} & \num{4.857} \\
Sample values & \num{3.641} & \num{4.362} & \num{4.517} & \num{4.730} & \num{4.805} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{3.610} & \num{4.480} & \num{4.725} & \num{5.198} & \num{5.377} \\
$\bm k = (2, 2, 2, 1)$ & \num{3.609} & \num{4.478} & \num{4.724} & \num{5.197} & \num{5.376} \\
$\bm k = (3, 3, 3, 1)$ & \num{3.610} & \num{4.480} & \num{4.725} & \num{5.198} & \num{5.377} \\
$\bm k = (4, 4, 4, 1)$ & \num{3.610} & \num{4.480} & \num{4.726} & \num{5.199} & \num{5.377} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.014} & \num{0.022} & \num{0.025} & \num{0.033} & \num{0.036} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.014} & \num{0.023} & \num{0.026} & \num{0.035} & \num{0.037} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.014} & \num{0.022} & \num{0.026} & \num{0.034} & \num{0.036} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.014} & \num{0.023} & \num{0.027} & \num{0.034} & \num{0.038} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.037} & \num{0.107} & \num{0.197} & \num{0.422} & \num{0.522} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.037} & \num{0.105} & \num{0.196} & \num{0.420} & \num{0.520} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.036} & \num{0.107} & \num{0.197} & \num{0.421} & \num{0.521} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.037} & \num{0.107} & \num{0.198} & \num{0.422} & \num{0.522} \\
\bottomrule 
\end{tabularx}


==> assets/GaussRevGamma/250/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,3.687[$ & 125 & 4 & 0.500 & 1.173 & 3.414 & 10.847 & 35.713 \\
2 & $[3.687,4.410[$ & 100 & 4 & 0.400 & 1.614 & 6.528 & 26.463 & 107.532 \\
3 & $[4.410,4.781[$ & 22 & 4 & 0.088 & 0.400 & 1.818 & 8.268 & 37.626 \\
4 & $[4.781,\infty[$ & 3 & 1 & 0.012 & 0.059 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/GaussRevGamma/250/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{3.643} & \num{4.376} & \num{4.530} & \num{4.778} & \num{4.857} \\
Sample values & \num{3.687} & \num{4.410} & \num{4.521} & \num{4.781} & \num{4.851} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{3.589} & \num{4.468} & \num{4.715} & \num{5.188} & \num{5.367} \\
$\bm k = (2, 2, 2, 1)$ & \num{3.589} & \num{4.468} & \num{4.714} & \num{5.189} & \num{5.368} \\
$\bm k = (3, 3, 3, 1)$ & \num{3.589} & \num{4.467} & \num{4.713} & \num{5.189} & \num{5.369} \\
$\bm k = (4, 4, 4, 1)$ & \num{3.589} & \num{4.469} & \num{4.715} & \num{5.189} & \num{5.366} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.054} & \num{0.049} & \num{0.051} & \num{0.057} & \num{0.060} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.054} & \num{0.049} & \num{0.051} & \num{0.058} & \num{0.060} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.054} & \num{0.048} & \num{0.050} & \num{0.056} & \num{0.059} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.054} & \num{0.048} & \num{0.050} & \num{0.056} & \num{0.059} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.077} & \num{0.105} & \num{0.192} & \num{0.414} & \num{0.514} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.077} & \num{0.104} & \num{0.191} & \num{0.415} & \num{0.514} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.077} & \num{0.103} & \num{0.190} & \num{0.415} & \num{0.515} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.077} & \num{0.105} & \num{0.191} & \num{0.414} & \num{0.513} \\
\bottomrule 
\end{tabularx}


==> assets/GaussRevGamma/500/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,3.677[$ & 250 & 4 & 0.500 & 1.189 & 3.481 & 11.065 & 36.388 \\
2 & $[3.677,4.419[$ & 200 & 4 & 0.400 & 1.612 & 6.510 & 26.362 & 107.023 \\
3 & $[4.419,4.750[$ & 45 & 4 & 0.090 & 0.410 & 1.869 & 8.519 & 38.850 \\
4 & $[4.750,\infty[$ & 5 & 1 & 0.010 & 0.048 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/GaussRevGamma/500/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{3.643} & \num{4.376} & \num{4.530} & \num{4.778} & \num{4.857} \\
Sample values & \num{3.677} & \num{4.419} & \num{4.562} & \num{4.750} & \num{4.801} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{3.606} & \num{4.482} & \num{4.728} & \num{5.202} & \num{5.382} \\
$\bm k = (2, 2, 2, 1)$ & \num{3.606} & \num{4.482} & \num{4.728} & \num{5.203} & \num{5.382} \\
$\bm k = (3, 3, 3, 1)$ & \num{3.606} & \num{4.481} & \num{4.727} & \num{5.203} & \num{5.383} \\
$\bm k = (4, 4, 4, 1)$ & \num{3.606} & \num{4.483} & \num{4.729} & \num{5.202} & \num{5.378} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.040} & \num{0.044} & \num{0.046} & \num{0.053} & \num{0.056} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.040} & \num{0.043} & \num{0.047} & \num{0.055} & \num{0.054} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.039} & \num{0.043} & \num{0.046} & \num{0.052} & \num{0.057} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.039} & \num{0.042} & \num{0.045} & \num{0.054} & \num{0.058} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.055} & \num{0.116} & \num{0.204} & \num{0.427} & \num{0.528} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.055} & \num{0.115} & \num{0.203} & \num{0.428} & \num{0.527} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.054} & \num{0.114} & \num{0.203} & \num{0.428} & \num{0.529} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.054} & \num{0.115} & \num{0.204} & \num{0.427} & \num{0.525} \\
\bottomrule 
\end{tabularx}


==> assets/LogNormal/1000/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,0.974[$ & 500 & 4 & 0.500 & 0.337 & 0.243 & 0.184 & 0.146 \\
2 & $[0.974,1.916[$ & 400 & 4 & 0.400 & 0.534 & 0.738 & 1.058 & 1.568 \\
3 & $[1.916,3.394[$ & 90 & 4 & 0.090 & 0.211 & 0.506 & 1.252 & 3.191 \\
4 & $[3.394,\infty[$ & 10 & 1 & 0.010 & 0.045 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/LogNormal/1000/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{1.000} & \num{1.898} & \num{2.276} & \num{3.200} & \num{3.625} \\
Sample values & \num{0.974} & \num{1.916} & \num{2.297} & \num{3.394} & \num{4.327} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.997} & \num{1.877} & \num{2.371} & \num{3.250} & \num{3.512} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.997} & \num{1.877} & \num{2.371} & \num{3.252} & \num{3.515} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.997} & \num{1.878} & \num{2.371} & \num{3.249} & \num{3.511} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.997} & \num{1.879} & \num{2.372} & \num{3.252} & \num{3.516} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.019} & \num{0.085} & \num{0.191} & \num{0.178} & \num{0.185} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.019} & \num{0.085} & \num{0.192} & \num{0.176} & \num{0.182} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.019} & \num{0.086} & \num{0.191} & \num{0.178} & \num{0.182} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.020} & \num{0.085} & \num{0.193} & \num{0.178} & \num{0.182} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.020} & \num{0.087} & \num{0.214} & \num{0.185} & \num{0.217} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.019} & \num{0.088} & \num{0.214} & \num{0.183} & \num{0.213} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.019} & \num{0.088} & \num{0.214} & \num{0.185} & \num{0.215} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.020} & \num{0.087} & \num{0.215} & \num{0.186} & \num{0.212} \\
\bottomrule 
\end{tabularx}


==> assets/LogNormal/2000/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,0.993[$ & 1000 & 4 & 0.500 & 0.348 & 0.258 & 0.201 & 0.162 \\
2 & $[0.993,1.867[$ & 800 & 4 & 0.400 & 0.533 & 0.733 & 1.041 & 1.524 \\
3 & $[1.867,3.309[$ & 180 & 4 & 0.090 & 0.205 & 0.476 & 1.136 & 2.786 \\
4 & $[3.309,\infty[$ & 20 & 1 & 0.010 & 0.044 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/LogNormal/2000/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{1.000} & \num{1.898} & \num{2.276} & \num{3.200} & \num{3.625} \\
Sample values & \num{0.993} & \num{1.867} & \num{2.210} & \num{3.309} & \num{4.125} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{1.002} & \num{1.882} & \num{2.365} & \num{3.244} & \num{3.512} \\
$\bm k = (2, 2, 2, 1)$ & \num{1.001} & \num{1.882} & \num{2.368} & \num{3.245} & \num{3.512} \\
$\bm k = (3, 3, 3, 1)$ & \num{1.001} & \num{1.881} & \num{2.364} & \num{3.241} & \num{3.511} \\
$\bm k = (4, 4, 4, 1)$ & \num{1.002} & \num{1.881} & \num{2.368} & \num{3.247} & \num{3.515} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.012} & \num{0.058} & \num{0.177} & \num{0.122} & \num{0.160} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.012} & \num{0.058} & \num{0.179} & \num{0.123} & \num{0.160} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.013} & \num{0.057} & \num{0.179} & \num{0.120} & \num{0.158} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.012} & \num{0.059} & \num{0.179} & \num{0.130} & \num{0.161} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.012} & \num{0.060} & \num{0.198} & \num{0.130} & \num{0.196} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.012} & \num{0.060} & \num{0.201} & \num{0.131} & \num{0.195} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.013} & \num{0.060} & \num{0.199} & \num{0.127} & \num{0.195} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.012} & \num{0.061} & \num{0.201} & \num{0.138} & \num{0.195} \\
\bottomrule 
\end{tabularx}


==> assets/LogNormal/250/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,1.010[$ & 125 & 4 & 0.500 & 0.346 & 0.258 & 0.203 & 0.166 \\
2 & $[1.010,1.779[$ & 100 & 4 & 0.400 & 0.519 & 0.694 & 0.959 & 1.366 \\
3 & $[1.779,3.537[$ & 22 & 4 & 0.088 & 0.198 & 0.459 & 1.093 & 2.694 \\
4 & $[3.537,\infty[$ & 3 & 1 & 0.012 & 0.052 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/LogNormal/250/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{1.000} & \num{1.898} & \num{2.276} & \num{3.200} & \num{3.625} \\
Sample values & \num{1.010} & \num{1.779} & \num{2.169} & \num{3.537} & \num{4.347} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{1.022} & \num{1.877} & \num{2.308} & \num{3.167} & \num{3.433} \\
$\bm k = (2, 2, 2, 1)$ & \num{1.021} & \num{1.877} & \num{2.308} & \num{3.173} & \num{3.436} \\
$\bm k = (3, 3, 3, 1)$ & \num{1.021} & \num{1.876} & \num{2.306} & \num{3.166} & \num{3.429} \\
$\bm k = (4, 4, 4, 1)$ & \num{1.021} & \num{1.877} & \num{2.307} & \num{3.169} & \num{3.434} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.033} & \num{0.110} & \num{0.272} & \num{0.438} & \num{0.464} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.033} & \num{0.112} & \num{0.275} & \num{0.442} & \num{0.471} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.033} & \num{0.110} & \num{0.273} & \num{0.440} & \num{0.468} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.033} & \num{0.112} & \num{0.272} & \num{0.442} & \num{0.469} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.039} & \num{0.111} & \num{0.274} & \num{0.439} & \num{0.502} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.039} & \num{0.113} & \num{0.277} & \num{0.442} & \num{0.507} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.039} & \num{0.113} & \num{0.275} & \num{0.441} & \num{0.507} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.040} & \num{0.114} & \num{0.274} & \num{0.443} & \num{0.507} \\
\bottomrule 
\end{tabularx}


==> assets/LogNormal/500/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,0.998[$ & 250 & 4 & 0.500 & 0.343 & 0.251 & 0.193 & 0.154 \\
2 & $[0.998,1.923[$ & 200 & 4 & 0.400 & 0.536 & 0.743 & 1.068 & 1.587 \\
3 & $[1.923,3.358[$ & 45 & 4 & 0.090 & 0.212 & 0.514 & 1.277 & 3.262 \\
4 & $[3.358,\infty[$ & 5 & 1 & 0.010 & 0.048 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/LogNormal/500/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{1.000} & \num{1.898} & \num{2.276} & \num{3.200} & \num{3.625} \\
Sample values & \num{0.998} & \num{1.923} & \num{2.259} & \num{3.358} & \num{4.137} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{1.006} & \num{1.909} & \num{2.401} & \num{3.249} & \num{3.494} \\
$\bm k = (2, 2, 2, 1)$ & \num{1.006} & \num{1.907} & \num{2.402} & \num{3.251} & \num{3.498} \\
$\bm k = (3, 3, 3, 1)$ & \num{1.005} & \num{1.908} & \num{2.400} & \num{3.246} & \num{3.492} \\
$\bm k = (4, 4, 4, 1)$ & \num{1.006} & \num{1.909} & \num{2.402} & \num{3.253} & \num{3.497} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.021} & \num{0.097} & \num{0.181} & \num{0.296} & \num{0.339} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.021} & \num{0.092} & \num{0.181} & \num{0.291} & \num{0.339} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.021} & \num{0.096} & \num{0.183} & \num{0.292} & \num{0.333} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.021} & \num{0.097} & \num{0.183} & \num{0.298} & \num{0.337} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.021} & \num{0.098} & \num{0.220} & \num{0.300} & \num{0.364} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.022} & \num{0.092} & \num{0.221} & \num{0.295} & \num{0.362} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.021} & \num{0.096} & \num{0.221} & \num{0.296} & \num{0.359} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.022} & \num{0.098} & \num{0.223} & \num{0.303} & \num{0.361} \\
\bottomrule 
\end{tabularx}


==> assets/LogNormal/750/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{1.000} & \num{1.898} & \num{2.276} & \num{3.200} & \num{3.625} \\
Sample values & \num{0.948} & \num{1.885} & \num{2.251} & \num{3.332} & \num{4.207} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{1.000} & \num{1.892} & \num{2.400} & \num{3.275} & \num{3.518} \\
$\bm k = (2, 2, 2, 1)$ & \num{1.000} & \num{1.890} & \num{2.401} & \num{3.277} & \num{3.520} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.999} & \num{1.891} & \num{2.399} & \num{3.276} & \num{3.517} \\
$\bm k = (4, 4, 4, 1)$ & \num{1.000} & \num{1.890} & \num{2.398} & \num{3.276} & \num{3.519} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.020} & \num{0.083} & \num{0.184} & \num{0.201} & \num{0.233} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.020} & \num{0.081} & \num{0.186} & \num{0.205} & \num{0.235} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.021} & \num{0.085} & \num{0.187} & \num{0.201} & \num{0.231} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.021} & \num{0.081} & \num{0.185} & \num{0.206} & \num{0.234} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.020} & \num{0.083} & \num{0.222} & \num{0.215} & \num{0.257} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.020} & \num{0.081} & \num{0.224} & \num{0.219} & \num{0.258} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.021} & \num{0.085} & \num{0.223} & \num{0.215} & \num{0.255} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.021} & \num{0.081} & \num{0.222} & \num{0.219} & \num{0.257} \\
\bottomrule 
\end{tabularx}


==> assets/MixGamma1/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,8.735[$ & 1000 & 4 & 0.500 & 2.948 & 18.667 & 124.806 & 869.766 \\
2 & $[8.735,32.491[$ & 800 & 4 & 0.400 & 8.230 & 199.368 & 5298.931 & 147776.551 \\
3 & $[32.491,41.574[$ & 180 & 4 & 0.090 & 3.215 & 115.277 & 4150.464 & 150050.700 \\
4 & $[41.574,\infty[$ & 20 & 1 & 0.010 & 0.438 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/MixNormalBeta/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,0.365[$ & 375 & 4 & 0.500 & 0.124 & 0.034 & 0.010 & 0.003 \\
2 & $[0.365,0.925[$ & 300 & 4 & 0.400 & 0.206 & 0.114 & 0.068 & 0.044 \\
3 & $[0.925,1.598[$ & 67 & 4 & 0.089 & 0.108 & 0.134 & 0.169 & 0.217 \\
4 & $[1.598,\infty[$ & 8 & 1 & 0.011 & 0.019 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/MixNormalBeta/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{0.366} & \num{1.000} & \num{1.225} & \num{1.548} & \num{1.653} \\
Sample values & \num{0.365} & \num{0.925} & \num{1.203} & \num{1.598} & \num{1.717} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.370} & \num{1.011} & \num{1.234} & \num{1.518} & \num{1.612} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.370} & \num{1.012} & \num{1.233} & \num{1.516} & \num{1.609} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.370} & \num{1.013} & \num{1.234} & \num{1.518} & \num{1.612} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.370} & \num{1.013} & \num{1.234} & \num{1.518} & \num{1.611} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.006} & \num{0.064} & \num{0.043} & \num{0.045} & \num{0.046} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.006} & \num{0.064} & \num{0.043} & \num{0.045} & \num{0.048} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.006} & \num{0.062} & \num{0.043} & \num{0.045} & \num{0.048} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.006} & \num{0.062} & \num{0.043} & \num{0.044} & \num{0.047} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.007} & \num{0.065} & \num{0.044} & \num{0.054} & \num{0.062} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.007} & \num{0.065} & \num{0.044} & \num{0.056} & \num{0.065} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.007} & \num{0.064} & \num{0.044} & \num{0.055} & \num{0.063} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.007} & \num{0.064} & \num{0.044} & \num{0.054} & \num{0.063} \\
\bottomrule 
\end{tabularx}


==> assets/ex1/problemtable.tex <==
\begin{tabularx}{\linewidth}{c|llllXXXX}
\toprule 
$j$ & $[b_{j-1},b_j[$ & $N_j$ & $k_j$ & $\pi_j$ & $\hat{\mu}_{j,1}$ & $\hat{\mu}_{j,2}$ & $\hat{\mu}_{j,3}$ & $\hat{\mu}_{j,4}$ \\
\midrule 
1 & $[0.000,0.998[$ & 250 & 4 & 0.500 & 0.343 & 0.251 & 0.193 & 0.154 \\
2 & $[0.998,1.923[$ & 200 & 4 & 0.400 & 0.536 & 0.743 & 1.068 & 1.587 \\
3 & $[1.923,3.358[$ & 45 & 4 & 0.090 & 0.212 & 0.514 & 1.277 & 3.262 \\
4 & $[3.358,\infty[$ & 5 & 1 & 0.010 & 0.048 &  &  &  \\
\bottomrule 
\end{tabularx}


==> assets/ex1/quantiles.tex <==
\begin{tabularx}{\linewidth}{c|XXXXX}
\toprule 
$\alpha$ & 0.5 & 0.9 & 0.95 & 0.99 & 0.995 \\
\midrule 
True values & \num{1.000} & \num{1.898} & \num{2.276} & \num{3.200} & \num{3.625} \\
Sample values & \num{0.998} & \num{1.923} & \num{2.259} & \num{3.358} & \num{4.137} \\
\midrule 
\multicolumn{1}{c}{Mean} \\
$\bm k = (1, 1, 1, 1)$ & \num{1.006} & \num{1.909} & \num{2.401} & \num{3.249} & \num{3.494} \\
$\bm k = (2, 2, 2, 1)$ & \num{1.006} & \num{1.907} & \num{2.402} & \num{3.251} & \num{3.498} \\
$\bm k = (3, 3, 3, 1)$ & \num{1.005} & \num{1.908} & \num{2.400} & \num{3.246} & \num{3.492} \\
$\bm k = (4, 4, 4, 1)$ & \num{1.006} & \num{1.909} & \num{2.402} & \num{3.253} & \num{3.497} \\
\midrule 
\multicolumn{1}{c}{Std} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.021} & \num{0.097} & \num{0.181} & \num{0.296} & \num{0.339} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.021} & \num{0.092} & \num{0.181} & \num{0.291} & \num{0.339} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.021} & \num{0.096} & \num{0.183} & \num{0.292} & \num{0.333} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.021} & \num{0.097} & \num{0.183} & \num{0.298} & \num{0.337} \\
\midrule 
\multicolumn{1}{c}{Rmse} \\
$\bm k = (1, 1, 1, 1)$ & \num{0.021} & \num{0.098} & \num{0.220} & \num{0.300} & \num{0.364} \\
$\bm k = (2, 2, 2, 1)$ & \num{0.022} & \num{0.092} & \num{0.221} & \num{0.295} & \num{0.362} \\
$\bm k = (3, 3, 3, 1)$ & \num{0.021} & \num{0.096} & \num{0.221} & \num{0.296} & \num{0.359} \\
$\bm k = (4, 4, 4, 1)$ & \num{0.022} & \num{0.098} & \num{0.223} & \num{0.303} & \num{0.361} \\
\bottomrule 
\end{tabularx}

